Ground Truth Or Dare: Factors Affecting The Creation Of Medical Datasets For Training AI

One of the core goals of responsible AI development is ensuring high-quality training datasets. Many researchers have pointed to the importance of the annotation step in the creation of high-quality data, but less attention has been paid to the work that enables data annotation. We define this work as the design of ground truth schema and explore the challenges involved in the creation of datasets in the medical domain even before any annotations are made. Based on extensive work in three health-tech organisations, we describe five external and internal factors that condition medical dataset creation processes. Three external factors include regulatory constraints, the context of creation and use, and commercial and operational pressures. These factors condition medical data collection and shape the ground truth schema design. Two internal factors include epistemic differences and limits of labelling. These directly shape the design of the ground truth schema. Discussions of what constitutes high-quality data need to pay attention to the factors that shape and constrain what is possible to be created, to ensure responsible AI design.

==> Tables/table-internal-1.tex <==
{\small
\begin{table*}
\caption{Internal}
\label{tab:internal}
\begin{tabular}{p{\textwidth}}
\toprule

% \textbf{Factor \ \ \ Arena}\\
% \midrule
\textbf{Epistemic Differences}
\begin{itemize}
    \item Misapprehension of technical knowledge by medical professionals may result in false assumptions and flawed design choices.
    \item During a labelling process that misapprehends medical practice, medical professionals are reconstructing their practice.
    \item Medical practice is misapprehended for the labelled data to meet quality requirements originating from data science.
    \item Medical knowledge is misapprehended to fit in a machine-learning model.
    \item Clinical diagnosis is never made based on a single source of information and it's always subjective.
\end{itemize}
\midrule
\textbf{Limits of Labelling}
\begin{itemize}
    \item Domain expert buy-in is crucial and may require concessions on the type and amount of collected data.
    \item Different than the usual distribution of x-rays while labelling induces overreporting of findings.
    \item Written and shallow in-person introductions to the labelling task reduce the chance for a "common mindset" among labellers.
    \item The labelling setup's physical limitations afflict the labelling quality.
    \item Experience and tacit knowledge support the use of clinical diagnoses without additional information.
    \item The UI of the labelling tool may influence the precision of the labels and induce overreporting.
    \item The selection and naming of the labels may influence a radiologist's read of an x-ray.
\end{itemize}
\bottomrule
\end{tabular}
\end{table*}
}


==> Tables/table-internal-2.tex <==
{\small
\begin{table}

\begin{tabular}{p{\linewidth}}
\toprule

\textbf{Epistemic differences}
\begin{itemize}
    \item Misapprehension of medical knowledge
    \item Misapprehension of medical practice
    \item Misunderstanding of technical knowledge
\end{itemize}

\midrule
\textbf{Limits of labelling}
\begin{itemize}
    \item Domain expert buy-in
    \item Different than the usual distribution of x-rays while labelling induces overreporting of findings when labelling a dataset .
    \item Written and shallow in-person introductions to the labelling task reduce the chance for a "common mindset" among labellers.
    \item The labelling setup's physical limitations afflict the labelling quality.
    \item Experience and tacit knowledge support the use of clinical diagnoses without additional information.
    \item The UI of the labelling tool may influence the precision of the labels and induce overreporting.
    \item The selection and naming of the labels may influence a radiologist's read of an x-ray.
\end{itemize}

\bottomrule
\end{tabular}
\caption{Internal factors}
\label{tab:internal}
\end{table}
}

==> Tables/table-internal-3.tex <==
{\small
\begin{table*}
\caption{Internal}
\label{tab:internal}
\begin{tabular}{p{\textwidth}}
\toprule

% \textbf{Factor \ \ \ Arena}\\
% \midrule
\textbf{Epistemic Differences}
\begin{itemize}
    \item Miscommunication and errors in translation between technical and medical domains may result in frustration, greater resource needs, and design choices made under flawed premises.
    \item A labelling process that misapprehends medical practice may result in medical professionals reconstructing their practice with inadequate resources.
    \item Prioritising computer science's notion of data quality may result in a misapprehension of medical practice.
    \item Prioritising machine learning data needs may result in a misapprehension of medical knowledge. 
\end{itemize}
\midrule
\textbf{Limits of Labelling}
\begin{itemize}
    \item Domain expert buy-in is crucial and may require concessions on the type and amount of collected data.
    \item Experience and tacit knowledge may help medical professionals label cases without contextual information.
    \item Written and superficial in-person onboarding to the labelling task may afflict the agreement between the annotators.
    \item Distribution of cases in the dataset different from the annotator's usual may result in overreporting of findings.
    \item The selection and naming of labels may influence how medical professionals interpret a case.
    \item The User Interface of a labelling tool may afflict the labelling quality and induce overreporting of findings.
    \item The labelling setup's physical limitations may afflict the labelling quality.
\end{itemize}
\bottomrule
\end{tabular}
\end{table*}
}


==> Tables/table-internal-4.tex <==
{\small
\begin{table*}
\caption{Internal}
\label{tab:internal}
\begin{tabular}{p{\textwidth}}
\toprule

% \textbf{Factor \ \ \ Arena}\\
% \midrule
\textbf{Epistemic Differences}
\begin{itemize}
    \item Miscommunication and errors in translation between technical and medical domains may result in frustration, greater resource needs, and design choices made under flawed premises.
    \item Prioritising computer science's notion of data quality may result in a misapprehension of medical practice.
    \item A labelling process that misapprehends medical practice may result in medical professionals reconstructing their practice with inadequate resources.
    \item Prioritising machine learning data needs may result in a misapprehension of medical knowledge. 
\end{itemize}
\midrule
\textbf{Limits of Labelling}
\begin{itemize}
    \item Domain expert buy-in is crucial and may require concessions on the type and amount of collected data.
    \item Experience and tacit knowledge may help medical professionals label cases without contextual information.
    \item Written and superficial in-person onboarding to the labelling task may afflict the agreement between the annotators.
    \item Distribution of cases in the dataset different from the annotator's usual may result in overreporting of findings.
    \item The selection and naming of labels may influence how medical professionals interpret a case.
    \item The User Interface of a labelling tool may afflict the labelling quality and induce overreporting of findings.
    \item The labelling setup's physical limitations may afflict the labelling quality.
\end{itemize}
\bottomrule
\end{tabular}
\end{table*}
}


==> Tables/table-participants-1.tex <==
{\small
\begin{table*}
% \caption{Participants. \\
% Role: R - Radiologist, ML - ML Engineer, B - Biomedical Engineer, MG - Project manager, HCI - HCI researcher \\ Experience: J < 5 years, 5 < M < 10 years, S > 10 years }
\caption{Tryout table for the Participants [NOT COMPLETE]}
\label{tab:participants}
\begin{tabular}{l l l l l}
\toprule
\textbf{Participants}   & \textbf{Position}                   & \textbf{Exp.}   & \textbf{Project} & \textbf{Participation} \\
\midrule
RJ1                 & Radiologist                         & \textless 5 y     & Project I        & Design Group         \\
RS2, RS4        & Radiologist                         & \textgreater 10 y & Project 1        & Design Group         \\
MLE1, MLE2, BE1 & ML, Biomedical Engineer  & \textgreater 5 y  & Project 1        & Design Group         \\
MG1                    & Project Manager, Computer Scientist & \textgreater 10 y & Project 1        & Design Group         \\
HCI1                    & HCI researcher                      & \textless 5 y     & Project 1        & Design Group         \\
HCI2                   & HCI researcher                      & \textgreater 15 y & Project 1        & Design Group         \\
RJ1N                 & Radiologist                         & \textless 5 y     & Project 1        & Evaluation           \\
RM1N, RM2N        & Radiologist                         & \textless 10 y    & Project 1        & Evaluation           \\
RS1N, RS3N, RS5S, RS6S, RS7S, RS8S, RS9S, RS10S & Radiologist & \textgreater 10 y & Project 1 & Evaluation \\

\bottomrule
\end{tabular}
\end{table*}
}
